Physical Effects in the Vicinity of Black Holes

General relativity, a theory that is already over a century old, is still the best theory that we have to describe the universe at energy scales where only the gravitational force is important. It has stood tall to any observational tests thrown at it since its inception, and it has remarkable predictive power when it is utilized to study and model astrophysical problems. It also continues to surprise us with its ability to generate new problems and insights that render themselves useful in the study of modern physics. This is especially highlighted by the transition of modern observational astronomy away from an electromagnetic radiation epoch, and into a new gravitational wave epoch. This thesis devotes its study to phenomena that can be analyzed within the framework of classical general relativity, but whose results may contain interesting implications for cosmological and black hole observations. (Full abstract can be found in document).

==> 00_LaTeX_Files/includeMacros.tex <==
%Tablularx Additional Column types (c,l,r work as normal)
	%Justified Auto-Width
		%Use a capitial 'X'
	%Centered Auto-Width
		\newcolumntype{C}{>{\centering\arraybackslash}X}
	%Left Justified Auto-Width
		\newcolumntype{L}{>{\raggedright\arraybackslash}X}
	%Right Justified Auto-Width
		\newcolumntype{R}{>{\raggedleft\arraybackslash}X}%

\renewcommand{\arraystretch}{1.5}


==> 00_LaTeX_Files/includePackages.tex <==
\usepackage[intoc]{nomencl}
	\makenomenclature
	\renewcommand\nomgroup[1]{%
		\item[\bfseries
		\ifstrequal{#1}{A}{Constants}{%
		\ifstrequal{#1}{B}{Latin}{%
		\ifstrequal{#1}{C}{Greek}{%
		\ifstrequal{#1}{D}{Subscripts}{}}}}]%
	}
	\renewcommand{\nomname}{List of Symbols}
	\newcommand{\nomunit}[1]{\renewcommand{\nomentryend}{\hspace*{\fill}#1}}

\usepackage[acronym,nonumberlist]{glossaries}
	\glstoctrue
	\makenoidxglossaries
	\newcommand{\addacronym}[2]{\newacronym{#1}{#1}{#2}}
	\newcommand{\addterm}[2]{\newglossaryentry{#1}{name={#1},description={#2}}}
	\newcommand\generateglossary{
		\printnoidxglossary[title={\glossaryname}]}
	\newcommand\abbreviations{
		\printnoidxglossary[type=\acronymtype,title={\abbreviationsname}]}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{enumitem}

% Provides the comment environment (Block Comments)
%   \begin{comment}
%       <Anything goes here>
%   \end{comment}
	\usepackage{comment} 

% The basics for using math in LaTeX
	\usepackage{array}
	\usepackage{amsmath}
	\usepackage{amsfonts}
	\usepackage{amssymb}

% Used to provide underlining that can be broken across multiple lines
	\usepackage[normalem]{ulem} 

% Used for creating subfigures
	\usepackage{subcaption}

% The defacto package for including graphics
	\usepackage{graphicx}

% Used to extend or replace the table/tabular environment
	\usepackage{tabularx}  % Auto-Sizing Tables
	\usepackage{xltabular} % Multi-page Tables
	\usepackage{pdflscape} % Allows creation of landscape pages
	\usepackage{booktabs}  % Nicer Lines
	\usepackage{multicol}  % Column Merging
	\usepackage{multirow}  % Row Merging
	\usepackage{makecell}  % Allows more control over cell contents

% Used for creating consistent plots and graphs
	\usepackage{pgfplots}
		\pgfplotsset{compat=newest}
		\usepgfplotslibrary{statistics, polar}
	\usepackage{pgf-pie}  % Adds Pie charts to PGF

% Allows the inclusion PDF files
	\usepackage{pdfpages}

% Used for inserting syntax highlighted code
	\usepackage{listings}

% Used for extending the rules/control for hyphenation
% \hyp{} allows the hyphenation of manually hyphenated Words: 
%   e.g. electromagnetic\hyp{}endioscopy
	\usepackage{hyphenat}

% Used for better quoting and formatting commands
	\usepackage{csquotes}
	\usepackage{ragged2e}

% Used for creating the Bibliography
%   Currently set up for 
%     - IEEE style citations
%     - Compact number in-text [1 - 3] vs [1, 2, 3]
%   To change the style to APA, MLA, or other change
%     - style=ieee, and remove the citestyle=numeric-comp
	\usepackage[
		style=ieee,
		citestyle=numeric-comp,
		dashed=false,
		backend=bibtex,
		refsegment=chapter,
		sorting=none,
		defernumbers=true]{biblatex}

% Used for including hyperlinks, document links, and better cross-references
	\usepackage{hyperref}
		\hypersetup{
			colorlinks,
			linkcolor={red!50!black},
			citecolor={blue!50!black},
			urlcolor={blue!80!black},
			pdfencoding=unicode,
			breaklinks=true
		}
		\urlstyle{same}
		\Urlmuskip=0mu plus 1mu\relax
	\usepackage[nameinlink]{cleveref} % Provides better/smarter cross-references
	\usepackage{xurl}                 % Fixes url line-breaking

% DELETE THE LINE AFTER THIS COMMENT, IT IS ONLY USED FOR THE GUIDE AND NOT 
%  NECESSARY FOR YOUR THESIS
	\input{./00_LaTeX_Files/guidePackages}

==> 00_LaTeX_Files/includeTheorems.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}
\newenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

==> 00_LaTeX_Files/listingCodeFormatting.tex <==
% Listings Code Formating
\lstdefinestyle{PropertyStyle}{
  language=HTML,
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=single,
  breaklines=true,
  basicstyle=\scriptsize,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[l][\color{orange!40!black}\ttfamily]{\#}
}

\lstdefinestyle{XMLStyle}{
  language=XML,
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=single,
  breaklines=true,
  basicstyle=\scriptsize,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[s][\color{green!40!black}\ttfamily]{<!--}{-->}
}

\lstdefinestyle{MatlabStyle}{
  language=Matlab,
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=single,
  breaklines=true,
  basicstyle=\scriptsize,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[s][\color{green!40!black}\ttfamily]{\%\{}{\%\}}
}

\lstdefinestyle{CStyle}{
  language=C,
  morekeywords={using,namespace},
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=single,
  breaklines=true,
  basicstyle=\scriptsize,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[l][\color{orange!40!black}\ttfamily]{\#},
  morecomment=[s][\color{green!40!black}\ttfamily]{/*}{*/}
}

\lstdefinestyle{VBStyle}{
  language=VBScript,
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=single,
  breaklines=true,
  basicstyle=\scriptsize,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[l][\color{orange!40!black}\ttfamily]{\#}
}

\lstdefinestyle{LaTeXStyle}{
  language=[LaTeX]{TeX},
  numbers=none,
  stepnumber=1,
  numbersep=12pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  frame=none,
  breaklines=true,
  moretexcs={Cref,cref,namecref,nameCref,autoref,cpageref,Cpageref,newcolumntype,arraybackslash,description,cmidrule,toprule,bottomrule,midrule,listofplates,tag,maketitle,vspace,hspace,chapter,subsection,geometry,degree,specialization,department,faculty,convocationdate,abstracttext,preface,thesisquote,dedication,acknowledgementtexts,subsubsection,paragraph,subparagraph,hfill,includegraphics,subfigure,includepdf,lstset,color,addplot},
  basicstyle=\normalsize\ttfamily,
  keywordstyle=\color{blue}\ttfamily,
  stringstyle=\color{magenta!80!red}\ttfamily,
  commentstyle=\color{green!40!black}\ttfamily,
  morecomment=[l][\color{orange!40!black}\ttfamily]{\#}
}

==> 00_LaTeX_Files/selectDegree.tex <==
Doctor of Philosophy
% Master of Science
% Master of Education
% Master of Business Administration
% Master of Accounting
% Master of Financial Management
% Master of Arts
% Master of Nursing
% Master of Laws
% Master of Music

==> 00_LaTeX_Files/selectDepartment.tex <==
% Department of Agricultural, Food and Nutritional Science
% Medical Science - Anaesthesia and Pain Medicine
% Department of Anthropology
% Department of Art and Design
% Department of Biochemistry
% Department of Biological Sciences
% Department of Biomedical Engineering
% Faculty of Business
% Department of Cell Biology
% Department of Chemical and Materials Engineering
% Department of Chemistry
% Department of Civil and Environmental Engineering
% Department of Comparative Literature
% Department of Computing Science
% Medical Sciences - Dentistry
% Department of Drama
% Department of Earth and Atmospheric Sciences
% Department of East Asian Studies
% Department of Economics
% Department of Educational Policy Studies
% Department of Educational Psychology
% Department of Educational Studies
% Department of Electrical and Computer Engineering
% Department of Elementary Education
% Department of English and Film Studies
% Faculty of Extension
% Health Promotion Studies
% Health Sciences Education
% Department of History and Classics
% Department of Human Ecology
% Humanities Computing
% Internetworking
% Medical Sciences - Laboratory Medicine and Pathology
% Department of Laboratory Medicine and Pathology
% Faculty of Law
% School of Library and Information Studies
% Department of Linguistics
% Department of Mathematical and Statistical Sciences
% Department of Mechanical Engineering
% Medical Sciences - Medical Genetics
% Department of Medical Microbiology and Immunology
% Department of Medicine
% Department of Modern Languages and Cultural Studies
% Department of Music
% Faculty of Native Studies
% Neuroscience
% Faculty of Nursing
% Medical Sciences - Obstetrics and Gynecology
% Department of Occupational Therapy
% Department of Oncology
% Medical Sciences - Ophthalmology
% Medical Sciences - Pediatrics
% Department of Pharmacology
% Faculty of Pharmacy and Pharmaceutical Sciences
% Department of Philosophy
% Faculty of Physical Education and Recreation
% Department of Physical Therapy
Department of Physics
% Department of Physiology
% Department of Political Science
% Department of Psychiatry
% Department of Psychology
% School of Public Health
% Department of Public Health Sciences
% Medical Sciences - Radiology and Diagnostic Imaging
% Department of Rehabilitation Science
% Department of Religious Studies
% Department of Renewable Resources
% Department of Resource Economics and Environmental Sociology
% Faculte\' Saint-Jean
% Department of Secondary Education
% Department of Sociology
% Department of Speech Pathology and Audiology
% Department of Surgery
% Department of Women's and Gender Studies

==> 01_Prefatory/Abstract.tex <==
\abstracttext{General relativity, a theory that is already over a century old, is still the best theory that we have to describe the universe at energy scales where only the gravitational force is important.  It has stood tall to any observational tests thrown at it since its inception, and it has remarkable predictive power when it is utilized to study and model astrophysical problems. It also continues to surprise us with its ability to generate new problems and insights that render themselves useful in the study of modern physics.  This is especially highlighted by the transition of modern observational astronomy away from an electromagnetic radiation epoch, and into a new gravitational wave epoch.

This thesis devotes its study to phenomena that can be analyzed within the framework of classical general relativity, but whose results may contain interesting implications for cosmological and black hole observations.  We can practically break the four main chapters of this thesis into three parts.  The first part details a procedure for Lorentz-boosting a general spacetime describing a compact rotating mass into the spacetime of a plane wave by taking the limit as the boost velocity approaches the speed of light.  This procedure creates a natural and mathematically trivial way to calculate scattering trajectories of null rays passing by a general compact rotating massive object.

The second part of this thesis, which is spanned by its third and fourth chapters, describes the evolution of a black hole's mass, velocity, and angular momentum as it travels through homogeneous scalar and electromagnetic fields.  For the case of the homogeneous scalar field, we allow it to take on a constant timelike, spacelike, or null gradient.  In some of these cases, the mass of the black hole can grow rapidly, and formally approach an infinite value, giving a possible mechanism for primordial black holes to become supermassive in the early universe. For the case of black holes traveling within homogeneous electromagnetic fields, we once again study the evolution of their parameters, this time finding that their mass cannot increase, and that their motion often resembles that of a charged particle in a homogeneous electromagnetic field.  This also offers implications of how black holes would evolve under the influence of strong primordial magnetic fields.

The final part of this thesis studies the propagation of high frequency electromagnetic waves as they are scattered by rotating black holes by taking higher order helicity-dependent corrections to the eikonal equation of the geometric optics approximation; this is known as the spinoptics approximation.  We derive a formalism to study the spinoptics approximation which recasts solving Maxwells equations in curved spacetime into studying the evolution of null rays and their associated null tetrads. These null tetrads correspond to the transport of polarized photons. We then derive a set of coupled differential equations describing the evolution for null rays and their associated tetrads that are scattered in the equatorial plane in the Kerr spacetime.  We extract an analytical approximation for scattering angles that are solely due to this spinoptics approximation, and show that it is small compared to the traditional scattering angles of null rays by Kerr black holes.  Lastly, further mechanisms associated with this effect are proposed and discussed.}

==> 01_Prefatory/Acknowledgements.tex <==
\acknowledgementtext{
I would first and foremost like to thank Professor Valeri Frolov for his guidance, wisdom, and mentoring throughout my time at the University of Alberta.  This thesis would not have been possible without his constant support and dedication to ensuring that I was prepared and trained from both an academic and professional standpoint.  His vibrant sense of humor was also important in maintaining my sanity throughout this process.  I would also like to extend a special thanks to Dr. Andrei Zelnikov, Dr. Jose Pinedo Soto, Prof. Don N. Page, and Prof. Saeed Rastgoo for their professional guidance and support.

Furthermore, I would like to thank the members of my doctoral examination committee, Prof. Don N. Page, Prof. Dmitri Pogosyan, Prof. Richard Sydora, and Prof. Sergey Sibiryakov for their time and care in reading my thesis.

Outside of the professional setting, I owe a massive debt of gratitude to my parents Denise and Philip Koek for raising me with love and care, and never doubting for a second my dream of pursuing a career in academia.  Similarly, I would like to thank my brother Sam Koek for his love and encouragement, and always being by my side.  In addition to this, I would like to thank my media naranja María Robles Hernandez for her extreme patience and support in being my better half, for making me a better and stronger person day-by-day, and for sharing the suffering that comes with being a doctoral student.

A special thanks to all my friends who were with me during my doctoral degree, including Dima Minchenko, Kalley Lasola, Dr. Brandon Chase, Paolo Fragolino, Artem Davydov, and Dunia Ajkal Valverde, among many other friends and family members.  To Dr. Jose Pinedo Soto, I would like to express my gratitude for being a companion and mentor throughout this whole endeavor, and taking me under his wing from the very start.
}

==> 01_Prefatory/Preface.tex <==
\preface{

I hereby declare that this Ph.D. thesis is the result of original research. All results presented herein were obtained using only the methods and sources explicitly stated, and all references have been properly cited.

This thesis is based on the following four publications: \cite{A1,A2,A3,A4}.  These works were carried out in close collaboration with Prof. Valeri Frolov.  The author of this thesis was actively involved in all aspects of these four research papers.  Chapters \ref{ch2}-\ref{ch5} each correspond to one of the papers referenced below in this preface.  Chapters \ref{ch1} and \ref{ch6} correspond to the introduction and conclusion of this thesis, respectively, and therefore offer a general look at the problem at hand.  Accordingly, they reference general results throughout this thesis as well as specific references mentioned therein.  Appendices~\ref{apxA}, \ref{apxB}, and \ref{apxC} offer supplemental calculations and discussion used throughout the thesis, as well as references that are mentioned specifically within the appendices themselves.

\begin{enumerate}
    \item V.P. Frolov and A. Koek, "Gravitational lensing, memory, and the Penrose limit," Phys. Rev. D 106 (2022) 064026.
    \item V.P. Frolov and A. Koek, "Motion of rotating black holes in homogeneous scalar fields: A general case," Phys. Rev. D 109 (2024) 084067.
    \item V.P. Frolov and A. Koek, "Motion of a weakly charged rotating black hole in a homogeneous electromagnetic field," Phys. Rev. D 110 (2024) 064052.
    \item V.P. Frolov and A. Koek, "Spinoptics in the Kerr spacetime: Polarized wave scattering," Phys. Rev. D 111 (2025) 104081.
\end{enumerate}

The following two papers \cite {A5,A6} are not part of this thesis, but also constitute research projects in which the author of this thesis was significantly involved at each step of investigation.  They were carried out in close collaboration with Prof. Valeri Frolov, as well as Dr. Andrei Zelnikov, and Dr. Jose Pinedo Soto.

\begin{enumerate}
    \item V.P. Frolov, A. Koek, J. Pinedo Soto, and A. Zelnikov, "Chiral anomalies in black hole spacetimes," Phys. Rev. D 107 (2023), no. 4 045009.
    \item V.P. Frolov, A. Koek, J. P. Soto, and A. Zelnikov, "Regular black holes inspired by quasitopological gravity," Phys. Rev. D 111 (2025), no. 4 044034.
\end{enumerate}
}

==> 01_Prefatory/Quotes_Dedications.tex <==
% Dedications, quotations, poems etc are optional. 
  % Ask your supervisor for advice or views on whether to include such matters in an academic work, with the next component serving as the place to thank people.
	\dedication{To María, el amor de mi vida}
